An External Stability Audit Framework to Test the Validity of Personality Prediction in AI Hiring

Automated hiring systems are among the fastest-developing of all high-stakes AI systems. Among these are algorithmic personality tests that use insights from psychometric testing, and promise to surface personality traits indicative of future success based on job seekers' resumes or social media profiles. We interrogate the validity of such systems using stability of the outputs they produce, noting that reliability is a necessary, but not a sufficient, condition for validity. Our approach is to (a) develop a methodology for an external audit of stability of predictions made by algorithmic personality tests, and (b) instantiate this methodology in an audit of two systems, Humantic AI and Crystal. Crucially, rather than challenging or affirming the assumptions made in psychometric testing -- that personality is a meaningful and measurable construct, and that personality traits are indicative of future success on the job -- we frame our methodology around testing the underlying assumptions made by the vendors of the algorithmic personality tests themselves. Our main contribution is the development of a socio-technical framework for auditing the stability of algorithmic systems. This contribution is supplemented with an open-source software library that implements the technical components of the audit, and can be used to conduct similar stability audits of algorithmic systems. We instantiate our framework with the audit of two real-world personality prediction systems, namely Humantic AI and Crystal. The application of our audit framework demonstrates that both these systems show substantial instability with respect to key facets of measurement, and hence cannot be considered valid testing instruments.

==> res/corr_tables_subgroup.tex <==

%%%% These tables take up about 8 pages and are not currently rendered.
%%%% They have not been highlighted. 
%%%% We also do not explain what DISC and OCEAEs stand for.


\onecolumn
\begin{table}[h!]
\caption{Rank-order stability of \crystal DiSC scores over file format and source context, as measured by Spearman's rank correlations. Reliabilities below 0.90 highlighted in yellow; those between 0.90 and 0.95 highlighted in lighter yellow. Results are discussed in Sections~\ref{sec:file_format_results}, \ref{sec:url_embedding_results}, \ref{sec:source_context_results}, \ref{sec:reproducibility_and_algorithm_time_results}, and \ref{sec:participant_time_results}.}
\label{crystal_corr_disc_fileformat_sourcecontext}
\begin{tabular}{>{\raggedright}p{0.14\textwidth} |>{\raggedright}p{0.2\textwidth} | >{\raggedright}p{0.08\textwidth} |>{\centering}p{0.02\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering\arraybackslash}p{0.05\textwidth}} 
\hline\noalign{\smallskip} Facet & Input Versions &   Group  & N &  D &  I &  S &  C \\
\noalign{\smallskip}\hline\noalign{\smallskip}
              File Format &   Raw Text Resume (CRr1) vs. PDF Resume (CRp1) &             All &  89 &     0.8225 &     0.8260 &      0.9184 &             0.9114 \\
              File Format &   Raw Text Resume (CRr1) vs. PDF Resume (CRp1) &            Male &  54 &     0.7628 &     0.8170 &      0.9460 &             0.9466 \\
              File Format &   Raw Text Resume (CRr1) vs. PDF Resume (CRp1) &          Female &  33 &     0.8805 &     0.8429 &      0.8883 &             0.8623 \\
              File Format &   Raw Text Resume (CRr1) vs. PDF Resume (CRp1) &         English &  56 &     0.8523 &     0.7900 &      0.8909 &             0.8864 \\
              File Format &   Raw Text Resume (CRr1) vs. PDF Resume (CRp1) &  Other Language &  33 &     0.7687 &     0.8688 &      0.9725 &             0.9570 \\
            Source Context &           PDF Resume (CRp1) vs. LinkedIn (CL1) &             All &  86 &     0.2335 &     0.5258 &      0.5103 &             0.3585 \\
            Source Context &           PDF Resume (CRp1) vs. LinkedIn (CL1) &            Male &  52 &     0.1092 &     0.4828 &      0.4571 &             0.2279 \\
            Source Context &           PDF Resume (CRp1) vs. LinkedIn (CL1) &          Female &  32 &     0.3375 &     0.5416 &      0.5297 &             0.4811 \\
            Source Context &           PDF Resume (CRp1) vs. LinkedIn (CL1) &         English &  55 &     0.1896 &     0.4638 &      0.4202 &             0.2509 \\
            Source Context &           PDF Resume (CRp1) vs. LinkedIn (CL1) &  Other Language &  31 &     0.4082 &     0.6678 &      0.6635 &             0.5612 \\
 
 \noalign{\smallskip}\hline
\end{tabular}
\end{table}

\begin{table}[h!]
\caption{Rank-order stability of \crystal DiSC scores over time, as measured by Spearman's rank correlations. Reliabilities below 0.90 highlighted in yellow; those between 0.90 and 0.95 highlighted in lighter yellow. Results are discussed in Sections~\ref{sec:file_format_results}, \ref{sec:url_embedding_results}, \ref{sec:source_context_results}, \ref{sec:reproducibility_and_algorithm_time_results}, and \ref{sec:participant_time_results}.}
\label{crystal_corr_disc_time}
\begin{tabular}{>{\raggedright}p{0.14\textwidth} |>{\raggedright}p{0.2\textwidth} | >{\raggedright}p{0.08\textwidth} |>{\centering}p{0.02\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering\arraybackslash}p{0.05\textwidth}} 
\hline\noalign{\smallskip} Facet & Input Versions &   Group  & N &  D &  I &  S &  C \\
\noalign{\smallskip}\hline\noalign{\smallskip}
 Immediate Reproducibility &   Raw Text Resume back-to-back (CRr2 vs. CRr3) &             All &  89 &     1.0000 &     1.0000 &      1.0000 &             1.0000 \\
 Immediate Reproducibility &   Raw Text Resume back-to-back (CRr2 vs. CRr3) &            Male &  54 &     1.0000 &     1.0000 &      1.0000 &             1.0000 \\
 Immediate Reproducibility &   Raw Text Resume back-to-back (CRr2 vs. CRr3) &          Female &  33 &     1.0000 &     1.0000 &      1.0000 &             1.0000 \\
 Immediate Reproducibility &   Raw Text Resume back-to-back (CRr2 vs. CRr3) &         English &  56 &     1.0000 &     1.0000 &      1.0000 &             1.0000 \\
 Immediate Reproducibility &   Raw Text Resume back-to-back (CRr2 vs. CRr3) &  Other Language &  33 &     1.0000 &     1.0000 &      1.0000 &             1.0000 \\
            Algorithm-Time &  Raw Text Resume 31 days apart (CRr1 vs. CRr2) &             All &  89 &     1.0000 &     1.0000 &      1.0000 &             1.0000 \\
            Algorithm-Time &  Raw Text Resume 31 days apart (CRr1 vs. CRr2) &            Male &  54 &     1.0000 &     1.0000 &      1.0000 &             1.0000 \\
            Algorithm-Time &  Raw Text Resume 31 days apart (CRr1 vs. CRr2) &          Female &  33 &     1.0000 &     1.0000 &      1.0000 &             1.0000 \\
            Algorithm-Time &  Raw Text Resume 31 days apart (CRr1 vs. CRr2) &         English &  56 &     1.0000 &     1.0000 &      1.0000 &             1.0000 \\
            Algorithm-Time &  Raw Text Resume 31 days apart (CRr1 vs. CRr2) &  Other Language &  33 &     1.0000 &     1.0000 &      1.0000 &             1.0000 \\
          Participant-Time &       LinkedIn 8-10 months apart (CL1 vs. CL2) &             All &  89 &     0.5314 &     0.7062 &      0.8676 &             0.7811 \\
          Participant-Time &       LinkedIn 8-10 months apart (CL1 vs. CL2) &            Male &  53 &     0.2316 &     0.6649 &      0.8537 &             0.7559 \\
          Participant-Time &       LinkedIn 8-10 months apart (CL1 vs. CL2) &          Female &  34 &     0.9326 &     0.8012 &      0.9138 &             0.8677 \\
          Participant-Time &       LinkedIn 8-10 months apart (CL1 vs. CL2) &         English &  57 &     0.5595 &     0.7189 &      0.8770 &             0.7703 \\
          Participant-Time &       LinkedIn 8-10 months apart (CL1 vs. CL2) &  Other Language &  32 &     0.4686 &     0.7169 &      0.8752 &             0.7874 \\
 \noalign{\smallskip}\hline
\end{tabular}
\end{table}

\begin{table}[h!]
\caption{Rank-order stability of \humantic DiSC scores over file format and URL embedding, as measured by Spearman's rank correlations. Reliabilities below 0.90 highlighted in yellow. Results are discussed in Sections~\ref{sec:file_format_results}, \ref{sec:url_embedding_results}, \ref{sec:source_context_results}, \ref{sec:reproducibility_and_algorithm_time_results}, and \ref{sec:participant_time_results}.}
\label{humantic_corr_disc_fileformat_url}
\begin{tabular}{>{\raggedright}p{0.14\textwidth} |>{\raggedright}p{0.2\textwidth} | >{\raggedright}p{0.08\textwidth} |>{\centering}p{0.02\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering\arraybackslash}p{0.05\textwidth}} 
\hline\noalign{\smallskip} Facet & Input Versions &   Group  & N &  D &  I &  S &  C \\
\noalign{\smallskip}\hline\noalign{\smallskip}
File Format &  De-Identified Resume (HRi1) vs. DOCX Resume (H... &             All &  89 &     0.9956 &     0.9924 &      0.9978 &                0.9959 \\
File Format &          De-Identified Resume (HRi1) vs. DOCX Resume (HRd1) &             All &  89 &     0.9956 &     0.9924 &      0.9978 &                0.9959 \\
               File Format &          De-Identified Resume (HRi1) vs. DOCX Resume (HRd1) &            Male &  54 &     0.9951 &     0.9944 &      0.9969 &                0.9941 \\
               File Format &          De-Identified Resume (HRi1) vs. DOCX Resume (HRd1) &          Female &  33 &     0.9931 &     0.9722 &      0.9946 &                0.9978 \\
               File Format &          De-Identified Resume (HRi1) vs. DOCX Resume (HRd1) &         English &  56 &     0.9966 &     0.9896 &      0.9965 &                0.9977 \\
               File Format &          De-Identified Resume (HRi1) vs. DOCX Resume (HRd1) &  Other Language &  33 &     0.9955 &     0.9945 &      0.9984 &                0.9927 \\
             URL Embedding &  URL-Embedded Resume (HRu1) vs. De-Identified Resume (HRi1) &             All &  86 &     0.3570 &     0.6253 &      0.5480 &                0.6878 \\
             URL Embedding &  URL-Embedded Resume (HRu1) vs. De-Identified Resume (HRi1) &            Male &  52 &     0.2549 &     0.7295 &      0.5745 &                0.7035 \\
             URL Embedding &  URL-Embedded Resume (HRu1) vs. De-Identified Resume (HRi1) &          Female &  32 &     0.4259 &     0.4860 &      0.4148 &                0.6706 \\
             URL Embedding &  URL-Embedded Resume (HRu1) vs. De-Identified Resume (HRi1) &         English &  55 &     0.3211 &     0.6706 &      0.5416 &                0.7512 \\
             URL Embedding &  URL-Embedded Resume (HRu1) vs. De-Identified Resume (HRi1) &  Other Language &  31 &     0.4753 &     0.5500 &      0.5646 &                0.5760 \\
             URL-Embedding &               URL-Embedded Resume (HRu1) vs. LinkedIn (HL1) &             All &  83 &     0.1555 &     0.3382 &      0.6074 &                0.4701 \\
             URL-Embedding &               URL-Embedded Resume (HRu1) vs. LinkedIn (HL1) &            Male &  50 &     0.1761 &     0.3642 &      0.5283 &                0.3872 \\
             URL-Embedding &               URL-Embedded Resume (HRu1) vs. LinkedIn (HL1) &          Female &  31 &     0.1621 &     0.2774 &      0.6985 &                0.5948 \\
             URL-Embedding &               URL-Embedded Resume (HRu1) vs. LinkedIn (HL1) &         English &  52 &     0.1217 &     0.4252 &      0.7253 &                0.5840 \\
             URL-Embedding &               URL-Embedded Resume (HRu1) vs. LinkedIn (HL1) &  Other Language &  31 &     0.1952 &     0.2156 &      0.3980 &                0.3051 \\
 \noalign{\smallskip}\hline
\end{tabular}
\end{table}

\begin{table}[h!]
\caption{Rank-order stability of \humantic DiSC scores, as measured by Spearman's rank correlations. Reliabilities below 0.90 highlighted in yellow. Results are discussed in Sections~\ref{sec:file_format_results}, \ref{sec:url_embedding_results}, \ref{sec:source_context_results}, \ref{sec:reproducibility_and_algorithm_time_results}, and \ref{sec:participant_time_results}.}
\label{humantic_corr_disc_sourcecontext}
\begin{tabular}{>{\raggedright}p{0.14\textwidth} |>{\raggedright}p{0.2\textwidth} | >{\raggedright}p{0.08\textwidth} |>{\centering}p{0.02\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering\arraybackslash}p{0.05\textwidth}} 
\hline\noalign{\smallskip} Facet & Input Versions &   Group  & N &  D &  I &  S &  C \\
\noalign{\smallskip}\hline\noalign{\smallskip}
Source Context &              De-Identified Resume (HRi1) vs. LinkedIn (HL1) &             All &  84 &     0.0903 &     0.2553 &      0.3941 &                0.3331 \\
            Source Context &              De-Identified Resume (HRi1) vs. LinkedIn (HL1) &            Male &  50 &     0.0972 &     0.2705 &      0.3501 &                0.3363 \\
            Source Context &              De-Identified Resume (HRi1) vs. LinkedIn (HL1) &          Female &  32 &     0.1922 &     0.3823 &      0.5106 &                0.3563 \\
            Source Context &              De-Identified Resume (HRi1) vs. LinkedIn (HL1) &         English &  52 &     0.0440 &     0.3795 &      0.5221 &                0.4502 \\
            Source Context &              De-Identified Resume (HRi1) vs. LinkedIn (HL1) &  Other Language &  32 &     0.1981 &     0.0245 &      0.1734 &                0.1209 \\
            Source Context &                   Original Resume (HRo1) vs. LinkedIn (HL1) &             All &  84 &     0.1775 &     0.4016 &      0.6939 &                0.6249 \\
            Source Context &                   Original Resume (HRo1) vs. LinkedIn (HL1) &            Male &  50 &     0.2597 &     0.3244 &      0.6584 &                0.4854 \\
            Source Context &                   Original Resume (HRo1) vs. LinkedIn (HL1) &          Female &  32 &     0.1317 &     0.6270 &      0.7385 &                0.7844 \\
            Source Context &                   Original Resume (HRo1) vs. LinkedIn (HL1) &         English &  52 &     0.1998 &     0.5713 &      0.7747 &                0.7356 \\
            Source Context &                   Original Resume (HRo1) vs. LinkedIn (HL1) &  Other Language &  32 &     0.1123 &     0.1628 &      0.5427 &                0.4749 \\
            Source Context &                    Original Resume (HRo1) vs. Twitter (HT1) &             All &  20 &    -0.5211 &     0.1026 &      0.0382 &               -0.1475 \\
            Source Context &                    Original Resume (HRo1) vs. Twitter (HT1) &            Male &  13 &    -0.4703 &     0.1114 &      0.0634 &               -0.1100 \\
            Source Context &                    Original Resume (HRo1) vs. Twitter (HT1) &          Female &   7 &    -0.5766 &     0.1441 &      0.0000 &               -0.2143 \\
            Source Context &                    Original Resume (HRo1) vs. Twitter (HT1) &         English &  16 &    -0.5100 &     0.1216 &     -0.0455 &               -0.2361 \\
            Source Context &                    Original Resume (HRo1) vs. Twitter (HT1) &  Other Language &   4 &    -0.4000 &     0.1054 &      0.8000 &                0.6000 \\
            Source Context &                            LinkedIn (HL1) vs. Twitter (HT1) &             All &  18 &    -0.1317 &     0.0203 &     -0.1120 &               -0.4329 \\
            Source Context &                            LinkedIn (HL1) vs. Twitter (HT1) &            Male &  11 &     0.2775 &    -0.0778 &      0.3396 &               -0.4838 \\
            Source Context &                            LinkedIn (HL1) vs. Twitter (HT1) &          Female &   7 &    -0.3214 &     0.3091 &     -0.6126 &               -0.0909 \\
            Source Context &                            LinkedIn (HL1) vs. Twitter (HT1) &         English &  15 &    -0.1562 &     0.0324 &     -0.0794 &               -0.3696 \\
            Source Context &                            LinkedIn (HL1) vs. Twitter (HT1) &  Other Language &   3 &     0.5000 &     0.0000 &     -0.5000 &               -1.0000 \\
\noalign{\smallskip}\hline
\end{tabular}
\end{table}

\begin{table}[h!]
\caption{Rank-order stability of \humantic DiSC scores over time, as measured by Spearman's rank correlations. Reliabilities below 0.90 highlighted in yellow. Results are discussed in Sections~\ref{sec:file_format_results}, \ref{sec:url_embedding_results}, \ref{sec:source_context_results}, \ref{sec:reproducibility_and_algorithm_time_results}, and \ref{sec:participant_time_results}.}
\label{humantic_corr_disc_time}
\begin{tabular}{>{\raggedright}p{0.14\textwidth} |>{\raggedright}p{0.2\textwidth} | >{\raggedright}p{0.08\textwidth} |>{\centering}p{0.02\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering\arraybackslash}p{0.05\textwidth}} 
\hline\noalign{\smallskip} Facet & Input Versions &   Group  & N &  D &  I &  S &  C \\
\noalign{\smallskip}\hline\noalign{\smallskip}
 Immediate Reproducibility &           De-Identified Resume back-to-back (HRi2 vs. HRi3) &             All &  89 &     0.9999 &     1.0000 &      1.0000 &                1.0000 \\
 Immediate Reproducibility &           De-Identified Resume back-to-back (HRi2 vs. HRi3) &            Male &  54 &     1.0000 &     1.0000 &      1.0000 &                1.0000 \\
 Immediate Reproducibility &           De-Identified Resume back-to-back (HRi2 vs. HRi3) &          Female &  33 &     0.9987 &     0.9999 &      1.0000 &                1.0000 \\
 Immediate Reproducibility &           De-Identified Resume back-to-back (HRi2 vs. HRi3) &         English &  56 &     0.9998 &     0.9999 &      1.0000 &                1.0000 \\
 Immediate Reproducibility &           De-Identified Resume back-to-back (HRi2 vs. HRi3) &  Other Language &  33 &     1.0000 &     1.0000 &      1.0000 &                1.0000 \\
            Algorithm-Time &          De-Identified Resume 31 days apart (HRi1 vs. HRi2) &             All &  89 &     0.9726 &     0.9948 &      0.9925 &                0.9980 \\
            Algorithm-Time &          De-Identified Resume 31 days apart (HRi1 vs. HRi2) &            Male &  54 &     0.9636 &     0.9992 &      0.9997 &                0.9988 \\
            Algorithm-Time &          De-Identified Resume 31 days apart (HRi1 vs. HRi2) &          Female &  33 &     0.9760 &     0.9774 &      0.9689 &                0.9944 \\
            Algorithm-Time &          De-Identified Resume 31 days apart (HRi1 vs. HRi2) &         English &  56 &     0.9990 &     0.9973 &      0.9994 &                0.9993 \\
            Algorithm-Time &          De-Identified Resume 31 days apart (HRi1 vs. HRi2) &  Other Language &  33 &     0.9458 &     0.9927 &      0.9828 &                0.9969 \\
          Participant-Time &                     LinkedIn 7-9 months apart (HL1 vs. HL2) &             All &  88 &     0.2248 &     0.4186 &      0.6597 &                0.5827 \\
          Participant-Time &                     LinkedIn 7-9 months apart (HL1 vs. HL2) &            Male &  52 &     0.1951 &     0.3601 &      0.5859 &                0.4782 \\
          Participant-Time &                     LinkedIn 7-9 months apart (HL1 vs. HL2) &          Female &  34 &     0.3760 &     0.4769 &      0.7222 &                0.6972 \\
          Participant-Time &                     LinkedIn 7-9 months apart (HL1 vs. HL2) &         English &  55 &     0.2018 &     0.5456 &      0.7467 &                0.6825 \\
          Participant-Time &                     LinkedIn 7-9 months apart (HL1 vs. HL2) &  Other Language &  33 &     0.2406 &     0.2222 &      0.4861 &                0.4499 \\
          Participant-Time &                      Twitter 7-9 months apart (HT1 vs. HT2) &             All &  21 &     1.0000 &     1.0000 &      1.0000 &                1.0000 \\
          Participant-Time &                      Twitter 7-9 months apart (HT1 vs. HT2) &            Male &  13 &     1.0000 &     1.0000 &      1.0000 &                1.0000 \\
          Participant-Time &                      Twitter 7-9 months apart (HT1 vs. HT2) &          Female &   8 &     1.0000 &     1.0000 &      1.0000 &                1.0000 \\
          Participant-Time &                      Twitter 7-9 months apart (HT1 vs. HT2) &         English &  17 &     1.0000 &     1.0000 &      1.0000 &                1.0000 \\
          Participant-Time &                      Twitter 7-9 months apart (HT1 vs. HT2) &  Other Language &   4 &     1.0000 &     1.0000 &      1.0000 &                1.0000 \\
\noalign{\smallskip}\hline
\end{tabular}
\end{table}

\begin{table}[h!]
\caption{Rank-order stability of \humantic Big Five scores over file format and URL embedding, as measured by Spearman's rank correlations. Reliabilities below 0.90 highlighted in yellow. Results are discussed in Sections~\ref{sec:file_format_results}, \ref{sec:url_embedding_results}, \ref{sec:source_context_results}, \ref{sec:reproducibility_and_algorithm_time_results}, and \ref{sec:participant_time_results}.}
\label{humantic_corr_big5_fileformat_url}
\begin{tabular}{>{\raggedright}p{0.14\textwidth} |>{\raggedright}p{0.2\textwidth} | >{\raggedright}p{0.08\textwidth} |>{\centering}p{0.02\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering\arraybackslash}p{0.05\textwidth}} 
\hline\noalign{\smallskip}
Facet & Input Versions &  Group & N &  O &  C &  E &  A &  ES \\
\noalign{\smallskip}\hline\noalign{\smallskip}
File Format &          De-Identified Resume (HRi1) vs. DOCX Resume (HRd1) &             All &  89 &    0.9891 &                      0.9936 &        0.9939 &         0.9927 &               0.9816 \\
               File Format &          De-Identified Resume (HRi1) vs. DOCX Resume (HRd1) &            Male &  54 &    0.9832 &                      0.9874 &        0.9920 &         0.9914 &               0.9838 \\
               File Format &          De-Identified Resume (HRi1) vs. DOCX Resume (HRd1) &          Female &  33 &    0.9948 &                      0.9954 &        0.9963 &         0.9967 &               0.9861 \\
               File Format &          De-Identified Resume (HRi1) vs. DOCX Resume (HRd1) &         English &  56 &    0.9921 &                      0.9975 &        0.9946 &         0.9902 &               0.9788 \\
               File Format &          De-Identified Resume (HRi1) vs. DOCX Resume (HRd1) &  Other Language &  33 &    0.9829 &                      0.9733 &        0.9936 &         0.9850 &               0.9850 \\
             URL Embedding &  URL-Embedded Resume (HRu1) vs. De-Identified Resume (HRi1) &             All &  86 &    0.3988 &                      0.3845 &        0.0772 &         0.4190 &               0.4040 \\
             URL Embedding &  URL-Embedded Resume (HRu1) vs. De-Identified Resume (HRi1) &            Male &  52 &    0.3957 &                      0.4525 &        0.1247 &         0.4755 &               0.4507 \\
             URL Embedding &  URL-Embedded Resume (HRu1) vs. De-Identified Resume (HRi1) &          Female &  32 &    0.3061 &                      0.2532 &       -0.0053 &         0.3540 &               0.3421 \\
             URL Embedding &  URL-Embedded Resume (HRu1) vs. De-Identified Resume (HRi1) &         English &  55 &    0.3056 &                      0.4248 &       -0.0273 &         0.3631 &               0.3803 \\
             URL Embedding &  URL-Embedded Resume (HRu1) vs. De-Identified Resume (HRi1) &  Other Language &  31 &    0.5037 &                      0.3389 &        0.2557 &         0.5098 &               0.3583 \\
             URL-Embedding &               URL-Embedded Resume (HRu1) vs. LinkedIn (HL1) &             All &  83 &    0.6381 &                      0.5470 &        0.5786 &         0.6839 &               0.7018 \\
             URL-Embedding &               URL-Embedded Resume (HRu1) vs. LinkedIn (HL1) &            Male &  50 &    0.5649 &                      0.4441 &        0.6283 &         0.6576 &               0.6534 \\
             URL-Embedding &               URL-Embedded Resume (HRu1) vs. LinkedIn (HL1) &          Female &  31 &    0.7019 &                      0.6333 &        0.4897 &         0.7465 &               0.8088 \\
             URL-Embedding &               URL-Embedded Resume (HRu1) vs. LinkedIn (HL1) &         English &  52 &    0.6501 &                      0.5691 &        0.5646 &         0.7227 &               0.7485 \\
             URL-Embedding &               URL-Embedded Resume (HRu1) vs. LinkedIn (HL1) &  Other Language &  31 &    0.6356 &                      0.5337 &        0.6286 &         0.5968 &               0.6547 \\
 \noalign{\smallskip}\hline
\end{tabular}
\end{table}

\begin{table}[h!]
\caption{Rank-order stability of \humantic Big Five scores over source context, as measured by Spearman's rank correlations. Reliabilities below 0.90 highlighted in yellow. Results are discussed in Sections~\ref{sec:file_format_results}, \ref{sec:url_embedding_results}, \ref{sec:source_context_results}, \ref{sec:reproducibility_and_algorithm_time_results}, and \ref{sec:participant_time_results}.}
\label{humantic_corr_big5_sourcecontext}
\begin{tabular}{>{\raggedright}p{0.14\textwidth} |>{\raggedright}p{0.2\textwidth} | >{\raggedright}p{0.08\textwidth} |>{\centering}p{0.02\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering\arraybackslash}p{0.05\textwidth}} 
\hline\noalign{\smallskip}
Facet & Input Versions &  Group & N &  O &  C &  E &  A &  ES \\
\noalign{\smallskip}\hline\noalign{\smallskip}
            Source Context &              De-Identified Resume (HRi1) vs. LinkedIn (HL1) &             All &  84 &    0.2180 &                      0.1558 &        0.1198 &         0.2020 &               0.2186 \\
            Source Context &              De-Identified Resume (HRi1) vs. LinkedIn (HL1) &            Male &  50 &    0.2885 &                      0.1459 &        0.1996 &         0.2247 &               0.1962 \\
            Source Context &              De-Identified Resume (HRi1) vs. LinkedIn (HL1) &          Female &  32 &    0.0557 &                      0.0473 &       -0.0414 &         0.2031 &               0.2874 \\
            Source Context &              De-Identified Resume (HRi1) vs. LinkedIn (HL1) &         English &  52 &    0.1573 &                      0.1614 &       -0.0398 &         0.1766 &               0.1596 \\
            Source Context &              De-Identified Resume (HRi1) vs. LinkedIn (HL1) &  Other Language &  32 &    0.2741 &                      0.0677 &        0.3529 &         0.3160 &               0.3108 \\
            Source Context &                   Original Resume (HRo1) vs. LinkedIn (HL1) &             All &  84 &    0.5985 &                      0.7124 &        0.5827 &         0.6136 &               0.5990 \\
            Source Context &                   Original Resume (HRo1) vs. LinkedIn (HL1) &            Male &  50 &    0.5978 &                      0.7338 &        0.6156 &         0.7466 &               0.6505 \\
            Source Context &                   Original Resume (HRo1) vs. LinkedIn (HL1) &          Female &  32 &    0.6086 &                      0.5726 &        0.4787 &         0.4389 &               0.5798 \\
            Source Context &                   Original Resume (HRo1) vs. LinkedIn (HL1) &         English &  52 &    0.5975 &                      0.7269 &        0.4816 &         0.5831 &               0.5925 \\
            Source Context &                   Original Resume (HRo1) vs. LinkedIn (HL1) &  Other Language &  32 &    0.6262 &                      0.7010 &        0.8128 &         0.7222 &               0.6115 \\
            Source Context &                    Original Resume (HRo1) vs. Twitter (HT1) &             All &  20 &   -0.1768 &                      0.2324 &       -0.1128 &        -0.2316 &               0.0692 \\
            Source Context &                    Original Resume (HRo1) vs. Twitter (HT1) &            Male &  13 &    0.0248 &                      0.4649 &       -0.1813 &        -0.3132 &               0.3187 \\
            Source Context &                    Original Resume (HRo1) vs. Twitter (HT1) &          Female &   7 &   -0.6071 &                     -0.2857 &        0.2143 &        -0.1786 &               0.0357 \\
            Source Context &                    Original Resume (HRo1) vs. Twitter (HT1) &         English &  16 &   -0.3441 &                      0.1280 &       -0.3176 &        -0.2941 &              -0.1412 \\
            Source Context &                    Original Resume (HRo1) vs. Twitter (HT1) &  Other Language &   4 &    0.0000 &                      0.4000 &        0.8000 &         0.4000 &               1.0000 \\
            Source Context &                            LinkedIn (HL1) vs. Twitter (HT1) &             All &  18 &   -0.2158 &                      0.0000 &       -0.1559 &        -0.1517 &              -0.1125 \\
            Source Context &                            LinkedIn (HL1) vs. Twitter (HT1) &            Male &  11 &   -0.0364 &                     -0.2232 &       -0.0091 &        -0.2000 &              -0.1364 \\
            Source Context &                            LinkedIn (HL1) vs. Twitter (HT1) &          Female &   7 &   -0.3214 &                      0.7143 &       -0.5000 &        -0.1071 &              -0.1429 \\
            Source Context &                            LinkedIn (HL1) vs. Twitter (HT1) &         English &  15 &   -0.3253 &                      0.1929 &       -0.3682 &        -0.3571 &              -0.1929 \\
            Source Context &                            LinkedIn (HL1) vs. Twitter (HT1) &  Other Language &   3 &   -0.5000 &                     -0.8660 &       -0.5000 &         0.5000 &              -0.5000 \\
 \noalign{\smallskip}\hline
\end{tabular}
\end{table}

\begin{table}[h!]
\caption{Rank-order stability of \humantic Big Five scores over time, as measured by Spearman's rank correlations. Reliabilities below 0.90 highlighted in yellow. Results are discussed in Sections~\ref{sec:file_format_results}, \ref{sec:url_embedding_results}, \ref{sec:source_context_results}, \ref{sec:reproducibility_and_algorithm_time_results}, and \ref{sec:participant_time_results}.}
\label{humantic_corr_big5_time}
\begin{tabular}{>{\raggedright}p{0.14\textwidth} |>{\raggedright}p{0.2\textwidth} | >{\raggedright}p{0.08\textwidth} |>{\centering}p{0.02\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering}p{0.05\textwidth} | >{\centering\arraybackslash}p{0.05\textwidth}} 
\hline\noalign{\smallskip}
Facet & Input Versions &  Group & N &  O &  C &  E &  A &  ES \\
\noalign{\smallskip}\hline\noalign{\smallskip}
Immediate Reproducibility &           De-Identified Resume back-to-back (HRi2 vs. HRi3) &             All &  89 &    1.0000 &                      1.0000 &        1.0000 &         0.9999 &               1.0000 \\
 Immediate Reproducibility &           De-Identified Resume back-to-back (HRi2 vs. HRi3) &            Male &  54 &    1.0000 &                      1.0000 &        1.0000 &         1.0000 &               1.0000 \\
 Immediate Reproducibility &           De-Identified Resume back-to-back (HRi2 vs. HRi3) &          Female &  33 &    1.0000 &                      1.0000 &        0.9999 &         1.0000 &               1.0000 \\
 Immediate Reproducibility &           De-Identified Resume back-to-back (HRi2 vs. HRi3) &         English &  56 &    1.0000 &                      1.0000 &        1.0000 &         1.0000 &               1.0000 \\
 Immediate Reproducibility &           De-Identified Resume back-to-back (HRi2 vs. HRi3) &  Other Language &  33 &    1.0000 &                      1.0000 &        1.0000 &         1.0000 &               1.0000 \\
            Algorithm-Time &          De-Identified Resume 31 days apart (HRi1 vs. HRi2) &             All &  89 &    0.9954 &                      0.9969 &        0.9618 &         0.9921 &               0.9854 \\
            Algorithm-Time &          De-Identified Resume 31 days apart (HRi1 vs. HRi2) &            Male &  54 &    0.9979 &                      0.9964 &        0.9719 &         0.9873 &               0.9976 \\
            Algorithm-Time &          De-Identified Resume 31 days apart (HRi1 vs. HRi2) &          Female &  33 &    0.9890 &                      0.9959 &        0.9527 &         0.9942 &               0.9594 \\
            Algorithm-Time &          De-Identified Resume 31 days apart (HRi1 vs. HRi2) &         English &  56 &    0.9976 &                      0.9994 &        0.9989 &         0.9985 &               0.9991 \\
            Algorithm-Time &          De-Identified Resume 31 days apart (HRi1 vs. HRi2) &  Other Language &  33 &    0.9935 &                      0.9947 &        0.9336 &         0.9809 &               0.9507 \\
          Participant-Time &                     LinkedIn 7-9 months apart (HL1 vs. HL2) &             All &  88 &    0.6879 &                      0.6928 &        0.7301 &         0.7518 &               0.7678 \\
          Participant-Time &                     LinkedIn 7-9 months apart (HL1 vs. HL2) &            Male &  52 &    0.6002 &                      0.6433 &        0.7618 &         0.7352 &               0.7095 \\
          Participant-Time &                     LinkedIn 7-9 months apart (HL1 vs. HL2) &          Female &  34 &    0.7710 &                      0.7127 &        0.6755 &         0.8049 &               0.8839 \\
          Participant-Time &                     LinkedIn 7-9 months apart (HL1 vs. HL2) &         English &  55 &    0.7178 &                      0.7107 &        0.7490 &         0.7730 &               0.8073 \\
          Participant-Time &                     LinkedIn 7-9 months apart (HL1 vs. HL2) &  Other Language &  33 &    0.6691 &                      0.6703 &        0.7128 &         0.7122 &               0.7165 \\
          Participant-Time &                      Twitter 7-9 months apart (HT1 vs. HT2) &             All &  21 &    1.0000 &                      1.0000 &        1.0000 &         1.0000 &               1.0000 \\
          Participant-Time &                      Twitter 7-9 months apart (HT1 vs. HT2) &            Male &  13 &    1.0000 &                      1.0000 &        1.0000 &         1.0000 &               1.0000 \\
          Participant-Time &                      Twitter 7-9 months apart (HT1 vs. HT2) &          Female &   8 &    1.0000 &                      1.0000 &        1.0000 &         1.0000 &               1.0000 \\
          Participant-Time &                      Twitter 7-9 months apart (HT1 vs. HT2) &         English &  17 &    1.0000 &                      1.0000 &        1.0000 &         1.0000 &               1.0000 \\
          Participant-Time &                      Twitter 7-9 months apart (HT1 vs. HT2) &  Other Language &   4 &    1.0000 &                      1.0000 &        1.0000 &         1.0000 &               1.0000 \\
 \noalign{\smallskip}\hline
\end{tabular}
\end{table}


\twocolumn

==> res/wilcoxon_tables_subgroup.tex <==
%%%% place holder for tables with subgroup p-values.
%%%% tables available at https://github.com/DataResponsibly/hiring-stability-audit/blob/main/analysis.ipynb
